On the minimum number of eigenvalues of trees of diameter seven

The underlying graph $G$ of a symmetric matrix $M=(m_{ij})\in \mathbb{R}^{n\times n}$ is the graph with vertex set $\{v_1,\ldots,v_n\}$ such that a pair $\{v_i,v_j\}$ with $i\neq j$ is an edge if and only if $m_{ij}\neq 0$. Given a graph $G$, let $q(G)$ be the minimum number of distinct eigenvalues in a symmetric matrix whose underlying graph is $G$. A symmetric matrix $M$ is said to be a realization of $q(G)$ if it has underlying graph $G$ and $q(G)$ distinct eigenvalues. In the case of trees, a paper by Johnson and Saiago [Johnson, C.R, and Saiago, C.M, Diameter Minimal Trees, Linear and Multilinear Algebra 64(3) (2015), 557--571.] proposed an approach by which realizations of large trees are constructed from realizations of smaller trees with the same diameter, known as seeds, which has proved to be very successful. In this paper, we discuss realizations of $q(T)$ for trees of diameter seven based on the seed that defines it, correcting a result in the aforementioned paper.

==> chap3-fig-under.tex <==

%\begin{figure}[h]
%\begin{svgraybox}
%\begin{programcode}{Tree diagonalization}
{\tt
\begin{tabbing}
aaa\=aaa\=aaa\=aaa\=aaa\=aaa\=aaa\=aaa\= \kill
     \> Input: matrix $M = (m_{ij})$ with underlying tree $T$\\
     \> Input: Bottom up ordering $v_1,\ldots,v_n$ of $V(T)$\\
     \> Input: real number $x$ \\
     \> Output: diagonal matrix $D = \mbox{diag}(d_1, \ldots, d_n)$ congruent to $M + xI$ \\
     \> \\
     \>  Algorithm $\mbox{Diagonalize}(M, x)$ \\
     \> \> initialize $d_i := m_{ii} + x$, for all $i$ \\
     \> \> {\bf for } $k = 1$ to $n$ \\
     \> \> \> {\bf if} $v_k$ is a leaf {\bf then} continue \\
     \> \> \> {\bf else if} $d_c \neq 0$ for all children $c$ of $v_k$ {\bf then} \\
     \> \> \>  \>   $d_k := d_k - \sum \frac{(m_{ck})^2}{d_c}$, summing over all children of $v_k$ \\
     \> \> \> {\bf else } \\
     \> \> \> \> select one child $v_j$ of $v_k$ for which $d_j = 0$  \\
     \> \> \> \> $d_k  := -\frac{(m_{jk})^2}{2}$ \\
     \> \> \> \> $d_j  :=  2$ \\
     \> \> \> \> if $v_k$ has a parent $v_\ell$, remove the edge $\{v_k,v_\ell\}$. \\
     \> \>  {\bf end loop} \\
\end{tabbing}
}
%%\end{programcode}
%\end{svgraybox}
%\caption{\label{treealgo} Diagonalizing $A + xI$.}
%\end{figure}



==> figure_new_seeds.tex <==
\begin{minipage}[h]{.24\textwidth}
\centering 
\begin{subfigure}{0.49\textwidth}
     %\includegraphics[width=\textwidth]{quad.png}
\centering 
\newseedtres   
     \caption{$S^{(3)}_{2k+4}$}
 \end{subfigure}
 
 \end{minipage}\hfill
\begin{minipage}[h]{.24\textwidth}
\centering

 \begin{subfigure}{0.49\textwidth}
     \centering
\newseedquatro    
\caption{$S^{(4)}_{2k+4}$}
 \end{subfigure}
 
 \end{minipage}
 \hfill
\begin{minipage}[h]{.24\textwidth}
\centering

 \begin{subfigure}{0.33\textwidth}
     \centering
        \newseedseis    
\caption{$S^{(5)}_{2k+4}$}
 \end{subfigure}
 
 \end{minipage}
  \hfill
\begin{minipage}[h]{.24\textwidth}
\centering

 \begin{subfigure}{0.33\textwidth}
     \centering
        \newseedcinco 
\caption{$S^{(6)}_{2k+4}$}
 \end{subfigure}
 
 \end{minipage}
